Structural constrained virtual histology staining for human coronary imaging using deep learning

Histopathological analysis is crucial in artery characterization for coronary artery disease (CAD). However, histology requires an invasive and time-consuming process. In this paper, we propose to generate virtual histology staining using Optical Coherence Tomography (OCT) images to enable real-time histological visualization. We develop a deep learning network, namely Coronary-GAN, to transfer coronary OCT images to virtual histology images. With a special consideration on the structural constraints in coronary OCT images, our method achieves better image generation performance than the conventional GAN-based method. The experimental results indicate that Coronary-GAN generates virtual histology images that are similar to real histology images, revealing the human coronary layers.

==> dummy.tex <==
\subsection{Threshold for camera moving filter}
\begin{figure}[h]
\centering
\includegraphics[width=8cm]{figures/CMFThreshold3.eps}
\caption{(a) The logarithm of mean sequence length over thresholds. After a threshold of 10000, all the frames pass the CMF. (b) The incremental of mean sequence length.}
\label{fig:CMFThreshold}
\end{figure}
Shorter but more stable video sequences are formulated by screening the MCCE dataset using CMF. The consecutive video frames that pass the CMF will be used for training the CNN+LSTM. We applied the CMF to the MCCE dataset and changed the threshold T. We plotted the resulting mean video sequence length against the threshold as shown in Figure \ref{fig:CMFThreshold}. With a higher threshold, the mean sequence length is longer as shown in Figure \ref{fig:CMFThreshold} (a). However, the selected video sequences contain more camera motion if we use higher thresholds. As shown in Figure \ref{fig:CMFThreshold} (b), the mean sequence length increases slower between [200, 800] compared to that of [0, 200]. Thus, a threshold of 200 is adopted for CMF in consideration of the trade-off between the sequence length and camera motion within sequences.
